Towards Improving Sequential Decision-Making in LLM Agents via Experience Memory

Large language models have improved substantially on single-shot reasoning tasks, but their performance in sequential decision-making is less well understood. We study this on fully-observable two-player zero-sum games, which provide ground-truth evaluation: outcomes are determined by the rules, and optimality of individual moves can be computed or approximated, without relying on a judge model. Across model tiers, LLMs play suboptimally in simple games such as tic-tac-toe or Connect Four, and lose to MCTS opponents. Obfuscations that preserve the game tree but rewrite its surface form leave performance largely unchanged, indicating the gap is not fully explained by recall of memorized strategies. Motivated by this performance gap, we introduce an agentic framework enhanced with an experience memory designed for the sequential setting and addressing common challenges of sequential decision-making such as credit assignment. We show that post-game reflection and rule extraction yield measurable improvements on tic-tac-toe without modifying the model weights.

==> shared.tex <==
% Shared macros for the IJCAI paper and accompanying TikZ diagrams.
% Define here any name or symbol that should stay consistent between
% the paper text and figure labels. Both ijcai26.tex and each diagram
% under ../diagrams/ may input this file.

\RequirePackage{xspace}

% Framework / system names
\providecommand{\omniplay}{PlyBench\xspace}
\providecommand{\recap}{REAPER\xspace}
\providecommand{\recapfull}{\textbf{R}eflective \textbf{E}xperiential \textbf{A}gent with \textbf{P}eriodic \textbf{E}xtraction of \textbf{R}ules\xspace}

% Tic-tac-toe family
\providecommand{\ttt}{tic-tac-toe\xspace}
\providecommand{\Ttt}{Tic-tac-toe\xspace}
\providecommand{\tttshort}{TTT\xspace}
\providecommand{\hid}{Hid\xspace}
\providecommand{\hidlong}{Hidden \ttt\xspace}
\providecommand{\msq}{M.Sq\xspace}
\providecommand{\msqlong}{Magic Square\xspace}
\providecommand{\msqadd}{M.Sq +$5$\xspace}
\providecommand{\msqaddlong}{Magic Square Add $5$\xspace}
\providecommand{\story}{Story\xspace}
\providecommand{\storylong}{Story Magic Square\xspace}

% Nim family
\providecommand{\nim}{Nim\xspace}
\providecommand{\nimhid}{Hid\xspace}
\providecommand{\nimhidlong}{Hidden Nim\xspace}
\providecommand{\niminv}{Inv\xspace}
\providecommand{\niminvlong}{Inverse Nim\xspace}
\providecommand{\nimstory}{Story\xspace}
\providecommand{\nimstorylong}{Story Nim\xspace}

% Connect Four
\providecommand{\cfour}{Connect Four\xspace}

% Algorithmic players and labels
\providecommand{\optimal}{Optimal\xspace}
\providecommand{\mcts}{MCTS\xspace}
\providecommand{\mctsfull}{Monte Carlo Tree Search\xspace}
\providecommand{\random}{Random\xspace}
\providecommand{\minimax}{Minimax\xspace}

% Generic phrasings
\providecommand{\sota}{state-of-the-art\xspace}
\providecommand{\efficient}{Efficient\xspace}
\providecommand{\intermediate}{Intermediate\xspace}
\providecommand{\frontier}{Frontier\xspace}

% Model names
\providecommand{\gptnano}{GPT-5 nano\xspace}
\providecommand{\gptmini}{GPT-5 mini\xspace}
\providecommand{\gpt}{GPT-5.4\xspace}
\providecommand{\geminiflold}{Gemini 2.5 Flash Lite\xspace}
\providecommand{\geminifold}{Gemini 2.5 Flash\xspace}
\providecommand{\geminifl}{Gemini 3.1 Flash Lite\xspace}
\providecommand{\geminif}{Gemini 3 Flash\xspace}
\providecommand{\gemini}{Gemini 3.1 Pro\xspace}
\providecommand{\glm}{GLM-5.2\xspace}
\providecommand{\oss}{GPT-OSS 120B\xspace}
\providecommand{\qwen}{Qwen 3.5 122B\xspace}

% Short model names
\providecommand{\gptnanoshort}{GPT-5 nano\xspace}
\providecommand{\gptminishort}{GPT-5 mini\xspace}
\providecommand{\gptshort}{GPT-5.4\xspace}
\providecommand{\geminifloldshort}{Gemini 2.5 FL\xspace}
\providecommand{\geminifoldshort}{Gemini 2.5 F\xspace}
\providecommand{\geminiflshort}{Gemini 3.1 FL\xspace}
\providecommand{\geminifshort}{Gemini 3 F\xspace}
\providecommand{\geminishort}{Gemini 3.1 Pro\xspace}
\providecommand{\glmshort}{GLM-5.2\xspace}
\providecommand{\ossshort}{GPT-OSS\xspace}
\providecommand{\qwenshort}{Qwen 3.5\xspace}

\providecommand{\original}{\textit{Original}\xspace}
\providecommand{\baseline}{\textit{Baseline}\xspace}

\newcommand{\wilson}{$95\%$ Wilson score confidence intervals\xspace}
\newcommand{\student}{$95\%$ Student's $t$ confidence intervals\xspace}

